Adversarially Robust Stability Certificates can be Sample-Efficient

Motivated by bridging the simulation to reality gap in the context of safety-critical systems, we consider learning adversarially robust stability certificates for unknown nonlinear dynamical systems. In line with approaches from robust control, we consider additive and Lipschitz bounded adversaries that perturb the system dynamics. We show that under suitable assumptions of incremental stability on the underlying system, the statistical cost of learning an adversarial stability certificate is equivalent, up to constant factors, to that of learning a nominal stability certificate. Our results hinge on novel bounds for the Rademacher complexity of the resulting adversarial loss class, which may be of independent interest. To the best of our knowledge, this is the first characterization of sample-complexity bounds when performing adversarial learning over data generated by a dynamical system. We further provide a practical algorithm for approximating the adversarial training algorithm, and validate our findings on a damped pendulum example.

==> backup.tex <==
Before we move on to establishing the generalization bounds, we first discuss our assumptions on the system dynamics.

\begin{assumption}[Stability in the sense of Lyapunov] \label{assumption: bounded adversary traj}
We assume there exists a compact set $S \subseteq \R^p$ such that $\varphi_t(\xi) \in S$ \emph{and} $\tvarphi_t(\xi) \in S$ for all $\xi \in X$, $t \in \calT$, where $\tvarphi$ comes from a given perturbation set $\Delta_\varepsilon(\xi)$.
\end{assumption}
For norm-bounded adversaries \eqref{def: norm-bounded pert ball}, this assumption is satisfied if, for example, the underlying nominal dynamics are input-to-state stable \citep{lin1995various}.  For Lipschitz \eqref{def: lipschitz-bounded pert ball} and combined \eqref{def: combo of adv} adversaries, additional care must be taken to ensure that $f(x) + \delta^x(x)$ remains input-to-state stable for all admissible $\delta^x(x)$.% that requires no further specification of what the perturbation set should look like, and includes all the previously described perturbation types, granted they fulfill the base assumption. 

We further make the following regularity assumptions on the certificate function:
\begin{assumption} \label{assumption: bounded constants}
We assume there exist constants $B_V$, $B_{\nabla V}$ such that
\begin{align*}
    &\sup_{V \in \calV} \sup_{x \in S} \abs{V(x)} \leq B_V \\
    &\sup_{V \in \calV} \sup_{x \in S} \norm{\nabla V(x)} \leq B_{\nabla V}.
\end{align*}
\end{assumption}
\Stephen{I think we should just develop everything for $\tilde{h}$ and state one lemma for its generalization (no need to replicate the nominal
arguments again)}
%
Given these boundedness assumptions, we define $L_V$ and $L_{\nabla V}$ as upper bounds on Lipschitz constants of the maps $x \mapsto V(x)$ and $x \mapsto \ip{\nabla V(x), f(x)}$ over $x \in S$. Given Assumptions~\ref{assumption: bounded adversary traj}, \ref{assumption: bounded constants}, the continuity of nominal dynamics $f(x)$, and the continuously differentiability of $V$, this implies that $L_V$ and $L_{\nabla V}$ are finite. We further define $B_h$ as the upper bound on $\sup_{V \in \calV} \sup_{x \in S}\abs{h(\xi, V)}$, and $L_h$ as the upper bound on the smoothness of the map
\begin{align*}
    (V, \nabla V) \mapsto \ip{\nabla V(x), f(x)} + \eta V(x)
\end{align*}
given any $x \in S$. $B_{\tildh}$ and $L_{\tildh}$ are defined similarly for the adversarial loss $\tildh(\xi, V)$. We then define the sup-norm on the space of certificate functions $\calV$
\begin{align*}
    \norm{V}_\calV = \sup_{x \in S} \norm{\bmat{V(x) \\ \nabla V(x)}},
\end{align*}
such that we have
\begin{equation}\label{eq: h to v-norm Lipschitz}
    \abs{h(\xi, V_1) - h(\xi, V_2)} \leq L_h \norm{V_1 - V_2}_\calV \quad \text{for all }\xi \in X,\; V_1,V_2 \in \calV.
\end{equation}
The key insight is to observe that any feasible solution $\hat{V}_n$ to \eqref{eq: empirical nominal feasibility} (respectively $\tilde{V}_n$ to \eqref{eq: empirical advrobust feasibility}) achieves zero empirical risk on the loss $\ell_n$ (resp. $\tilde{\ell}_n$):
\begin{align*}
    \ell_n(V) := \frac{1}{n}\sum_{i=1}^n \bone \curly{h(\xi_i, V) > -\tau}, \:\: \tilde{\ell}_n(V) := \frac{1}{n} \sum_{i=1}^n \bone \curly{\tilde{h}(\xi_i, V) > -\tau}.
\end{align*}
Therefore, results from statistical learning theory regarding zero empirical risk minimizers can be applied to get fast rates for the generalization error. To do so, we define the nominal and adversarial loss classes
\[
    \calH = \curly{h(\cdot, V), \; V \in \calV}, \quad \tilde{\calH} = \curly{\tilde{h}(\cdot, V),\; V \in \calV}.
\]
Lemma 4.1 from \cite{boffi2020learning}, which is in turn adapted from Theorem 5 of \cite{srebro2010smoothness}, gives the following bound on the generalization error in the nominal case.
\begin{lemma}\label{lem: nominal gen error}
    Fix a $\delta \in (0,1)$. Let us assume Assumptions~\ref{assumption: bounded adversary traj} and \ref{assumption: bounded constants}. Suppose that the optimization problem \eqref{eq: empirical nominal feasibility} is feasible and $\hat{V}_n$ is a solution. Then the following holds with probability at least $1-\delta$ over $\xi_1,\dots,\xi_n$ drawn i.i.d.\ from $\calD$:
    \begin{align}\label{eq: nominal gen bound}
        \err\paren{\hat{V}_n} \leq K \paren{\frac{\log^3(n)}{\tau^2} \calR_n^2(\calH) + \frac{2 \log\paren{\log\paren{4B_h/\tau}/\delta}}{n}},
    \end{align}
    where $K > 0$ is a universal constant and 
    \[
    \calR_n(\calH) := \sup_{\xi_1,\dots, \xi_n \in \calX} \Ex_{\sigma \sim \mathrm{Unif}\curly{\pm 1}^n}\brac{ \sup_{h(\cdot, \calV) \in \calH} \frac{1}{n} \abs{\sum_{i=1}^n \sigma_i h(\xi_i, V)}},
    \]
    is the Rademacher complexity of the nominal loss class $\calH$.
    
\end{lemma}
Once the loss class $\calH$ and related constants are given, it can be verified that the bound is agnostic to the problem specifications. In other words, the same generalization bound in Lemma~\ref{lem: nominal gen error} holds when we substitute $\tilde{V}_n$ and $\tilde{\calH}$ into it:
\begin{corollary}\label{cor: advrobust gen bound}
    Fix a $\delta \in (0,1)$. Let us assume Assumptions~\eqref{assumption: bounded adversary traj} and \eqref{assumption: bounded constants}. Suppose that the optimization problem \eqref{eq: empirical advrobust feasibility} is feasible and $\tilde{V}_n$ is a solution. Then the following holds with probability at least $1-\delta$ over $\xi_1,\dots,\xi_n$ drawn i.i.d.\ from $\calD$:
    \begin{align}\label{eq: adv gen bound}
        \err\paren{\tilde{V}_n} \leq K \paren{\frac{\log^3(n)}{\tau^2} \calR_n^2(\tilde{\calH}) + \frac{2 \log\paren{\log\paren{4B_{\tildh}/\tau}/\delta}}{n}},
    \end{align}
    where $K > 0$ is a universal constant and is the Rademacher complexity of the adversarially loss class $\tilde{\calH}$.
    
\end{corollary}
Therefore, Corollary~\ref{cor: advrobust gen bound} reduces bounding the generalization error of an adversarially robust stability certificate to bounding the Rademacher complexity of the adversarial loss class $\tilde{\calH}$.

